SALAD-Bench: A Hierarchical and Comprehensive Safety Benchmark for Large Language Models

In the rapidly evolving landscape of Large Language Models (LLMs), ensuring robust safety measures is paramount. To meet this crucial need, we propose \emph{SALAD-Bench}, a safety benchmark specifically designed for evaluating LLMs, attack, and defense methods. Distinguished by its breadth, SALAD-Bench transcends conventional benchmarks through its large scale, rich diversity, intricate taxonomy spanning three levels, and versatile functionalities.SALAD-Bench is crafted with a meticulous array of questions, from standard queries to complex ones enriched with attack, defense modifications and multiple-choice. To effectively manage the inherent complexity, we introduce an innovative evaluators: the LLM-based MD-Judge for QA pairs with a particular focus on attack-enhanced queries, ensuring a seamless, and reliable evaluation. Above components extend SALAD-Bench from standard LLM safety evaluation to both LLM attack and defense methods evaluation, ensuring the joint-purpose utility. Our extensive experiments shed light on the resilience of LLMs against emerging threats and the efficacy of contemporary defense tactics. Data and evaluator are released under https://github.com/OpenSafetyLab/SALAD-BENCH.

==> sections/related_work_short.tex <==
\section{Related works}
\label{sec:related_work}

Our SALAD-Bench are highly related to three aspects, \emph{i.e.}, safety evaluation datasets, large language models (LLMs), and corresponding attacka and defense approaches. 

\textcolor{blue}{(bowen: summarize existing works here, as short as possible, but should be accurate, to ensure the logic of this paper.)}

% With the advancement of LLM, there is a significant increase in safety concerns. These arise primarily due to the models' enhanced ability to produce text indistinguishable from that written by humans. This capability, while impressive, also opens doors for potential misuse. Consequently, safety research must evolve in tandem with the development of LLMs to address these concerns effectively.


% \subsection{LLM Safety dataset.}
% Although there are some datasets generated for toxic detection or bias detection~\citep{bolddataset,realtoxicprompts,toxigen}, the safety evaluation datasets are rare. Our comparison with the existing LLM safety datasets are shown in Table~\ref{datasets}.

% \subsection{Attack \& defense}
% \paragraph{Attack.} Attacks on LLMs typically aim to elicit harmful or undesirable responses, a phenomenon often referred to as "jailbreaking."~\citep{jailbreak-prompt0,gptfuzzer,multilingual}. Recent literature has explored various aspects of this issue. For instance, some studies focus on manually crafted jailbreak prompts~\citep{doanything} or red-teaming~\citep{}, often sourced from online platforms like jailbreakchat.com, Reddit or by careful human design. Others develop algorithms capable of automatically generating such prompts~\citep{gptfuzzer,autodan}. Among the algorithms, they can be classified into search based~\citep{20queries, treeofattack}, gradient based~\citep{universalattack} and transformation~\citep{Jailbroken}. Notably, GCG~\citep{universalattack} proposed a method for creating adversarial suffixes to elicit affirmative responses from LLMs. Building upon this, AutoDan~\citep{autodan} introduced an interpretable algorithm that not only generates attack prompts but also potentially exposes the underlying system prompts of LLMs. Another noteworthy approach is PAIR~\citep{20queries}, which creates semantic jailbreaks with only black-box access to an LLM by searching, demonstrating the diversity and complexity of attack strategies.


% \paragraph{Defense.}
% In contrast to the rapid progress in jailbreak attack methodologies, defensive strategies for LLMs have not been as extensively explored. Some research, like the work presented in~\citet{baselinedefense}, investigates various defensive tactics, such as the use of perplexity filters for preprocessing, paraphrasing input prompts, and adversarial training. While heuristic detection methods show promise, adversarial training has proven impractical due to the high computational costs involved in retraining LLMs. Another innovative approach is proposed in~\citet{certifyingllm}, which offers certifiable robustness through the application of safety filters on input prompt sub-strings. However, the complexity of this method increases with the length of the prompt, making it less feasible for longer inputs.~\citet{smoothllm} introduces a novel technique that involves perturbing and aggregating predictions from multiple variations of an input prompt to identify adversarial inputs, adding to the spectrum of potential defensive strategies.

% \subsection{Evaluation methods.}$@$dongbowen \& $@$ huxuhao
% Existing methods for evaluating the harmfulness or toxicity of the model's response can be roughly classified into the following 3 categories: (1)methods based on closed moderation classifiers APIs, such as Perspective API~\citep{perspective} and OpenAI Moderation API~\citep{openaimoderation}. Although they are well-maintained, they focus solely on toxic and harmful content, lacking sufficient coverage in terms of safety dimensions. (2)Method based on keyword detection is the second category which predefined a set of keywords such as "I'm sorry". It has been used in GCG~\citep{universalattack} which defines about 50 detection keywords. This method necessitates customizing distinct keywords for different models, and it is prone to a substantial number of false positives and false negatives. (3) LLMs as safety referees is the third category and possibly the most widely used and powerful method. This approach typically requires the careful design of prompts to instruct a powerful language model, often ChatGPT or GPT-4, as they are widely recognized for their superior capabilities, which is crucial for a referee model. Although this method has been used in ~\citet{gptfinetune}, ~\citet{donotanswer}, ~\citet{gptfuzzer}, and so on, it faces issues typical of black-box models, such as lack of control, limited reproducibility, and potential future loss of model checkpoint.

% However, the latest published safety check guard~\citep{inan2023llama} proposed a possibly valid approach: finetuning language model as a safeguard. In this way, we could customize the specific content that we want the safeguard model to generate, which is extensible and flexible.


